Optimal Control of Complex Systems through Variational Inference with a Discrete Event Decision Process

Complex social systems are composed of interconnected individuals whose interactions result in group behaviors. Optimal control of a real-world complex system has many applications, including road traffic management, epidemic prevention, and information dissemination. However, such real-world complex system control is difficult to achieve because of high-dimensional and non-linear system dynamics, and the exploding state and action spaces for the decision maker. Prior methods can be divided into two categories: simulation-based and analytical approaches. Existing simulation approaches have high-variance in Monte Carlo integration, and the analytical approaches suffer from modeling inaccuracy. We adopted simulation modeling in specifying the complex dynamics of a complex system, and developed analytical solutions for searching optimal strategies in a complex network with high-dimensional state-action space. To capture the complex system dynamics, we formulate the complex social network decision making problem as a discrete event decision process. To address the curse of dimensionality and search in high-dimensional state action spaces in complex systems, we reduce control of a complex system to variational inference and parameter learning, introduce Bethe entropy approximation, and develop an expectation propagation algorithm. Our proposed algorithm leads to higher system expected rewards, faster convergence, and lower variance of value function in a real-world transportation scenario than state-of-the-art analytical and sampling approaches.

==> camera ready/tmp.tex <==
%Discrete Event Model

A discrete event model is used to specify the complex system dynamics
with a sequence of stochastic events that each event changes the states
minimally, but when aggregated together, induces as complex as possible
system evolutions. Specifically, a discrete event model describes
the temporal evolution of a system with $M$ species $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots,X^{(M)}\}$
driven by $V$ mutually independent events parameterized by rate coefficients
$\mathbf{c}=(c_{1},\dots,c_{V})$. At any specific time $t$, the
populations of the species are $x_{t}=(x_{t}^{(1)},\dots,x_{t}^{(M)})$.
An event $v$ is specified as: \vspace{-4mm}

\begin{align}
 & \alpha_{v}^{(1)}X^{(1)}+\cdots+\alpha_{v}^{(M)}X^{(M)}\to\beta_{v}^{(1)}X^{(1)}+\cdots+\beta_{v}^{(M)}X^{(M)},\label{eq:reaction-1}\\
 & \text{with rate }h_{v}(x,c_{v})=c_{v}g_{v}(x)=c_{v}\prod_{m=1}^{M}g_{v}^{(m)}(x^{(m)}),\nonumber \\
 & \Delta_{v}=(\beta_{v}^{(1)}-\alpha_{v}^{(1)},\cdots,\beta_{v}^{(M)}-\alpha_{v}^{(M)}).\nonumber 
\end{align}

Eq. (\ref{eq:reaction-1}) details that when $\alpha_{v}^{(1)}$ individuals
of species $X^{(1)}$, $\alpha_{v}^{(2)}$ individuals of species
$X^{(2)}$, etc., react, they trigger event $v$ with rate coefficient
$c_{v}$, which result in $\beta_{v}^{(1)}$ individuals of species
$X^{(1)}$, $\beta_{v}^{(2)}$ individuals of species $X^{(2)}$,
and so on. Event $v$ changes the populations by $\Delta_{v}$ and
occurs at rate $h_{v}(x,c_{v})$. Event rate $h_{v}(x,c_{v})$ equals
to the rate constant $c_{v}$ times a total of $\prod_{m=1}^{M}g_{v}^{(m)}(x^{(m)})$
different ways for the individuals to react, where the formulation
of $h_{v}(x,c_{v})$ comes from the formulations of the stochastic
kinetic model and stochastic petri net \cite{xu2016using,wilkinson2011stochastic}. 

A discrete event model defines a discrete event process, also called
a Markov jump process. A discrete event process initially in state
$x_{0}$ at time $t=0$ can be simulated through (1) sampling the
event $v\in\left\{ \emptyset,1,\cdots,V\right\} $ according to categorical
distribution $v\sim(1-h_{0},h_{1},\dots,h_{V})$, where $h_{v}(x,c_{v})$
is the rate of event $v$ and $h_{0}(x,c)=\sum_{v=1}^{V}h_{v}(x,c_{v})$
is the rate of all events, and (2) updating the network state deterministically
$x\leftarrow x+\Delta_{v}$, until the termination condition is satisfied.
In a complex system, each event involves only a few state and action
variables. This generative process thus assigns a probabilistic measure
to a sample path induced by a sequence of events $v_{0},\dots,v_{T}$
happening between times $0,1,\cdots,T$, where $\delta$ is an indicator
function. \vspace{-4mm}

\begin{align*}
 & P(x_{0:T},v_{0:T})=p(x_{0})\prod_{t=0}^{T}p(v_{t}|x_{t})\delta_{x_{t+1}=x_{t}+\Delta_{v_{t}}},\\
 & \text{where }\\
 & p(v_{t}|x_{t})=\begin{cases}
1-h_{0}(x_{t},c)=1-\sum\nolimits _{v=1}^{V}h_{v}(x_{t},c_{v}), & v_{t}=\emptyset\\
h_{k}(x_{t},c_{k})=c_{k}\prod_{m=1}^{M}g_{k}^{(m)}(x_{t}^{(m)}), & v_{t}=k,
\end{cases}
\end{align*}

Discrete event model is a widely used model for social scientists
to specify complex network interaction dynamics \cite{marsan1994modelling,goss1998quantitative,forrester1997industrial,borshchev2013big}.
Some recent literatures \cite{yang2017integrating,fang2017expectation}
have also applied this model to inferring hidden state of complex systems.
But this model has not been explored in complex network intervention
and decision making. 






==> tmp.tex <==
%Discrete Event Model

A discrete event model is used to specify the complex system dynamics
with a sequence of stochastic events that each event changes the states
minimally, but when aggregated together, induces as complex as possible
system evolutions. Specifically, a discrete event model describes
the temporal evolution of a system with $M$ species $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots,X^{(M)}\}$
driven by $V$ mutually independent events parameterized by rate coefficients
$\mathbf{c}=(c_{1},\dots,c_{V})$. At any specific time $t$, the
populations of the species are $x_{t}=(x_{t}^{(1)},\dots,x_{t}^{(M)})$.
An event $v$ is specified as: \vspace{-4mm}

\begin{align}
 & \alpha_{v}^{(1)}X^{(1)}+\cdots+\alpha_{v}^{(M)}X^{(M)}\to\beta_{v}^{(1)}X^{(1)}+\cdots+\beta_{v}^{(M)}X^{(M)},\label{eq:reaction-1}\\
 & \text{with rate }h_{v}(x,c_{v})=c_{v}g_{v}(x)=c_{v}\prod_{m=1}^{M}g_{v}^{(m)}(x^{(m)}),\nonumber \\
 & \Delta_{v}=(\beta_{v}^{(1)}-\alpha_{v}^{(1)},\cdots,\beta_{v}^{(M)}-\alpha_{v}^{(M)}).\nonumber 
\end{align}

Eq. (\ref{eq:reaction-1}) details that when $\alpha_{v}^{(1)}$ individuals
of species $X^{(1)}$, $\alpha_{v}^{(2)}$ individuals of species
$X^{(2)}$, etc., react, they trigger event $v$ with rate coefficient
$c_{v}$, which result in $\beta_{v}^{(1)}$ individuals of species
$X^{(1)}$, $\beta_{v}^{(2)}$ individuals of species $X^{(2)}$,
and so on. Event $v$ changes the populations by $\Delta_{v}$ and
occurs at rate $h_{v}(x,c_{v})$. Event rate $h_{v}(x,c_{v})$ equals
to the rate constant $c_{v}$ times a total of $\prod_{m=1}^{M}g_{v}^{(m)}(x^{(m)})$
different ways for the individuals to react, where the formulation
of $h_{v}(x,c_{v})$ comes from the formulations of the stochastic
kinetic model and stochastic petri net \cite{xu2016using,wilkinson2011stochastic}. 

A discrete event model defines a discrete event process, also called
a Markov jump process. A discrete event process initially in state
$x_{0}$ at time $t=0$ can be simulated through (1) sampling the
event $v\in\left\{ \emptyset,1,\cdots,V\right\} $ according to categorical
distribution $v\sim(1-h_{0},h_{1},\dots,h_{V})$, where $h_{v}(x,c_{v})$
is the rate of event $v$ and $h_{0}(x,c)=\sum_{v=1}^{V}h_{v}(x,c_{v})$
is the rate of all events, and (2) updating the network state deterministically
$x\leftarrow x+\Delta_{v}$, until the termination condition is satisfied.
In a complex system, each event involves only a few state and action
variables. This generative process thus assigns a probabilistic measure
to a sample path induced by a sequence of events $v_{0},\dots,v_{T}$
happening between times $0,1,\cdots,T$, where $\delta$ is an indicator
function. \vspace{-4mm}

\begin{align*}
 & P(x_{0:T},v_{0:T})=p(x_{0})\prod_{t=0}^{T}p(v_{t}|x_{t})\delta_{x_{t+1}=x_{t}+\Delta_{v_{t}}},\\
 & \text{where }\\
 & p(v_{t}|x_{t})=\begin{cases}
1-h_{0}(x_{t},c)=1-\sum\nolimits _{v=1}^{V}h_{v}(x_{t},c_{v}), & v_{t}=\emptyset\\
h_{k}(x_{t},c_{k})=c_{k}\prod_{m=1}^{M}g_{k}^{(m)}(x_{t}^{(m)}), & v_{t}=k,
\end{cases}
\end{align*}

Discrete event model is a widely used model for social scientists
to specify complex network interaction dynamics \cite{marsan1994modelling,goss1998quantitative,forrester1997industrial,borshchev2013big}.
Some recent literatures \cite{yang2017integrating,fang2017expectation}
have also applied this model to inferring hidden state of complex systems.
But this model has not been explored in complex network intervention
and decision making. 





